Unveiling the Origin of GRB 090709A: Lack of Periodicity in a Reddened Cosmological Long-Duration Gamma-Ray Burst

We present broadband (gamma-ray, X-ray, near-infrared, optical, and radio) observations of the gamma-ray burst (GRB) 090709A and its afterglow in an effort to ascertain the origin of this high-energy transient. Previous analyses suggested that GRB 090709A exhibited quasi-periodic oscillations with a period of 8.06 s, a trait unknown in long-duration GRBs but typical of flares from soft gamma-ray repeaters. When properly accounting for the underlying shape of the power-density spectrum of GRB 090709A, we find no conclusive (> 3 sigma) evidence for the reported periodicity. In conjunction with the location of the transient (far from the Galactic plane and absent any nearby host galaxy in the local universe) and the evidence for extinction in excess of the Galactic value, we consider a magnetar origin relatively unlikely. A long-duration GRB, however, can account for the majority of the observed properties of this source. GRB 090709A is distinguished from other long-duration GRBs primarily by the large amount of obscuration from its host galaxy (A_K,obs >~ 2 mag).

==> obs.tab.tex <==
\ProvidesFile{obs.tab}

\begin{deluxetable*}{lcccccc}
  \tabletypesize{\scriptsize}
  \tablecaption{Optical/NIR Observations of GRB\,090709A}
  \tablecolumns{7}
  \tablewidth{0pc}
  \tablehead{\colhead{Observation Date} & \colhead{Time Since
             Burst\tablenotemark{a}} & \colhead{Telescope} & \colhead{Filter} &
             \colhead{Exposure Time} & \colhead{Magnitude\tablenotemark{b}} &
             \colhead{Reference} \\
             \colhead{(2009 UT)} & \colhead{(s)} & & & \colhead{(s)} & &
            }
  \startdata
    Jul 9 07:40:22 & 120.0 & PAIRITEL & $H$ & 23.4 & $15.52 \pm 0.16$ &
     * \\
    Jul 9 07:40:22 & 120.0 & PAIRITEL & $K_{s}$ & 23.4 & $14.48 \pm 0.21$ &
     * \\
    Jul 9 07:40:26 & 142.5 & P60 & $r^{\prime}$ & 60.0 & $21.80 \pm 0.51$ &
     * \\
    Jul 9 07:40:58 & 177.0 & PAIRITEL & $H$ & 46.8 & $> 15.90$ & * \\
    Jul 9 07:40:58 & 177.0 & PAIRITEL & $K_{s}$ & 46.8 & $14.25 \pm 0.14$ &
     * \\
    Jul 9 07:42:17 & 307.5 & PAIRITEL & $H$ & 117.0 & $16.20 \pm 0.13$ &
     * \\
    Jul 9 07:42:17 & 307.5 & PAIRITEL & $K_{s}$ & 117.0 & $15.00 \pm 0.15$ &
     * \\
    Jul 9 07:43:17 & 313.2 & P60 & $z^{\prime}$ & 60.0 & $19.54 \pm 0.30$ &
     * \\
    Jul 9 07:40:58 & 383.5 & PAIRITEL & $J$ & 304.2 & $18.43 \pm 0.28$ &
     * \\
    Jul 9 07:43:53 & 398.7 & P60 & $r^{\prime}$ & 180.0 & $22.24 \pm 0.42$ &
     * \\
    Jul 9 07:45:08 & 484.0 & P60 & $i^{\prime}$ & 180.0 & $> 21.62$ & * \\
    Jul 9 07:46:33 & 569.4 & P60 & $z^{\prime}$ & 180.0 & $> 19.92$ & * \\
    Jul 9 07:45:20 & 680.0 & PAIRITEL & $H$ & 351.0 & $16.88 \pm 0.16$ &
     * \\
    Jul 9 07:45:20 & 680.0 & PAIRITEL & $K_{s}$ & 351.0 & $15.89 \pm 0.21$ &
     * \\
    Jul 9 07:46:07 & $1.637 \times 10^{3}$ & FTN & $i^{\prime}$ & 520.0 &
     $> 20.6$ & 1 \\
    Jul 9 07:41:16 & $1.737 \times 10^{3}$ & FTN & $R$ & 720.0 & 
     $22.7 \pm 0.5$ & 1 \\
    Jul 9 08:06:34 & $2.040 \times 10^{3}$ & P60 & $r^{\prime}$ &
     720.0 & $> 22.81$ & * \\
    Jul 9 08:11:06 & $2.251 \times 10^{3}$ & P60 & $i^{\prime}$ & 600.0 & 
     $> 22.36$ & * \\
    Jul 9 08:13:11 & $2.377 \times 10^{3}$ & P60 & $z^{\prime}$ & 600.0 &  
     $> 20.75$ & * \\
    Jul 9 08:20:17 & $2.743 \times 10^{3}$ & P60 & $g^{\prime}$ &
     480.0 & $> 22.09$ & * \\
    Jul 9 09:30:00 & $6.686 \times 10^{3}$ & Subaru / MOIRCS & $K$ & 
     $\ldots$ & 18.2 & 2 \\
    Jul 9 22:37:55 & $5.479 \times 10^{4}$ & NOT / ALFOSC & $R$ & 1800.0 &
     $> 24.0$ & 3 \\
    Jul 9 23:46:42 & $6.488 \times 10^{4}$ & CAHA / OMEGA$_{2000}$ & $H$ &
     3600.0 & $> 20.73$ & * \\
    Jul 10 00:48:09 & $6.777 \times 10^{4}$ & CAHA / OMEGA$_{2000}$ & 
     $K_{s}$ & 4140.0 & $20.77 \pm 0.39$ & * \\
    Jul 10 01:57:43 & $6.801 \times 10^{4}$ & CAHA / OMEGA$_{2000}$ &
     $J$ & 3120.0 & $> 21.74$ & * \\
    Jul 11 00:45:00 & $1.480 \times 10^{5}$ & GTC / OSIRIS & $i^{\prime}$ &
     2100.0 & $> 25.5$ & * \\
    Jul 17 10:06:16 & $7.009 \times 10^{5}$ & Keck II / NIRC2 & 
     $K^{\prime}$ & 1500.0 & $> 22.81$ & * \\ 
  \enddata
  \tablenotetext{a}{Time elapsed from the \swift-BAT trigger, 07:38:34 
    UT on 9 July 2009 to the midpoint of the exposure.}
  \tablenotetext{b}{Magnitudes are provided in the AB system \citep{og83} for the 
    $g^{\prime}r^{\prime}i^{\prime}z^{\prime}$ filters and in the Vega system
    for the remaining filters.  Errors quoted are 1$\sigma$ photometric
    and instrumental errors summed in quadrature.  For measurements with
    significance $< 2\sigma$, 3$\sigma$ upper limits are provided.
    Galactic extinction ($E(B-V) = 0.09$\,mag; \citealt{sfd98}) has 
    not been incorporated in the reported magnitudes.}
  \tablerefs{* = this work; 1 = \citet{GCN.9648}; 2 = \citet{GCN.9634};
    3 = \citet{GCN.9644}.}
\label{tab:obs}
\end{deluxetable*}    


==> others.tab.tex <==
\ProvidesFile{others.tab}

\begin{deluxetable}{lcccc}[tb]
  \tabletypesize{\footnotesize}
  \tablecaption{Power Density Spectra of Bright \swift-BAT GRBs}
  \tablecolumns{5}
  \tablewidth{0pc}
  \tablehead{\colhead{GRB} & \colhead{Period\tablenotemark{a}} & \colhead{White 
             SNR\tablenotemark{b}} & \colhead{PDS Slope} & 
             \colhead{Red SNR\tablenotemark{c}} \\
             & \colhead{(s)} & \colhead{($\sigma$)} & & \colhead{($\sigma$)}
            }
  \startdata
    090709A & 8.1 & 14.1 & $-2.5$ & 5.0 \\
    \hline
    041223 & 16.5 & 2.0 & $-2.6$ & 0.4 \\
    061007 & 7.6 & 4.8 & $-2.2$ & 1.2 \\
    080319B & 8.3 & 4.6 & $-2.3$ & 0.8 \\
    080607 & 7.7 & 7.3 & $-2.2$ & 2.7 \\
    090201 & 8.3 & 8.8 & $-1.9$ & 3.5 \\
    090618 & 15.2 & 3.1 & $-2.2$ & 1.2 \\
  \enddata
  \tablenotetext{a}{Period of the strongest feature observed in the PDS.}
  \tablenotetext{b}{Single-trial signal-to-noise ratio of the strongest feature 
                    observed in the PDS assuming a flat (white) intrinsic
		    spectrum across the entire frequency range (normalized to
		    the region $P = 3$--6.5\,s).}
  \tablenotetext{c}{Single-trial signal-to-noise ratio of the strongest feature 
  		    observed in the PDS assuming an intrinsic power-law spectrum
                    (red noise).  See text for details.}
\label{tab:others}
\end{deluxetable}    

